One-Way Functions Imply Secure Computation in a Quantum World

We prove that quantum-hard one-way functions imply simulation-secure quantum oblivious transfer (QOT), which is known to suffice for secure computation of arbitrary quantum functionalities. Furthermore, our construction only makes black-box use of the quantum-hard one-way function. Our primary technical contribution is a construction of extractable and equivocal quantum bit commitments based on the black-box use of quantum-hard one-way functions in the standard model. Instantiating the Cr\'epeau-Kilian (FOCS 1988) framework with these commitments yields simulation-secure QOT.

==> sec-quantum-sampling.tex <==
\section{Proof of~\cref{lemma:quantum-sampling}}
\label{appendix:sampling}

We give a proof of~\cref{lemma:quantum-sampling}, which we restate here for convenience.

Consider the following interaction between a challenger and an unbounded quantum receiver $\cR$ (initialized with an arbitrary quantum ``advice'' state):
\begin{enumerate}
\item The challenger generates $k$ EPR pairs and sends one half of each to a receiver.
\item The receiver $\cR$ replies with $k$-bit strings $\hat{\theta}, \hat{x}$ purported to be the results of measuring these EPR pairs in bases specified by $\hat{\theta}$.
\item The challenger picks a random subset $T$ (of size $t$) of $[k]$ and measures its halves of the corresponding EPR pairs in the bases dictated by $\hat{\theta}_T$. The interaction is deemed \emph{successful} if the measurement outcomes correspond with $\hat{x}_T$.
\item Define $\overline{T} \coloneqq [k] \setminus T$ and let $n \coloneqq |\overline{T}|$. If the interaction has been successful, the challenger samples a random $n$-bit string $\theta$ and measures its $n$ remaining EPR states in the bases specified by $\theta$, obtaining measurement outcomes $x_T$.
\end{enumerate}

\begin{lemma}[Quantum Sampling]
Let $\brho$ be the quantum state of any successful receiver $\cR$ in the above interaction. Then for any $\epsilon > 0$, we have
\[ \mathbf{H}_{\infty}(x_T \mid \brho) \geq \frac{(1-\epsilon)t}{2}\]
with probability $1-\negl$ \fermi{fill in the negligible} (over the randomness of $\theta$).
\end{lemma}



\subsection{The~\cite{C:BouFeh10} EPR Protocol}

We describe a protocol we call the ``EPR Protocol,'' which is essentially equivalent to the ``QOT*'' protocol described by~\cite{C:BouFeh10}. This protocol is exclusively stated as a tool for arguing about the security of BB84-style protocols, and should not be viewed as a functional protocol.

In the EPR protocol, party $A$ deviates from the standard BB84-style template, instead generating EPR pairs and sending one half of each pair. From the other party's point of view, this message is distributed identically to random BB84 states, since in both cases each qubit is maximally mixed. Note that in a standard BB84-style protocol, $A$ samples a random bit string $x$ and encodes it in a random bases before interacting with $B$. But in the EPR protocol, $A$ obtains $x$ as the result of measuring her halves of the EPR pairs; this has the advantage of significantly simplifying arguments about the entropy of $x$ from $B$'s point of view~\cite{C:BouFeh10}. 

This is captured in~\cref{lemma:min-entropy}, which relies heavily on quantum sampling techniques of~\cite{C:BouFeh10}.

\protocol
{\proref{fig:epr-protocol}}
{EPR Protocol.}
{fig:epr-protocol}
{

\textbf{Parameters:} $m = n+k$. 

\begin{enumerate}
\item $A$ prepares $m$ EPR pairs and sends one of each pair to $B$. $A$ also samples $\theta \gets \{+,\times\}^m$.

\item $B$ responds with $\widehat{\theta} \in \{+,\times\}^m,\widehat{x} \in \{0,1\}^m$.

\item $A$ sends a random test subset $T \subset [m]$ of size $k$.

\item $B$ responds with either continue or abort.

\item $A$ measures each of her qubits in $T$ in the corresponding basis of $\widehat{\theta}$. For any index $i$ such that $\widehat{\theta}_i = \theta_i$, $A$ checks that the measured $x_i$ matches $\widehat{x}_i$. If not, $A$ aborts. If all checks pass, $A$ restricts her qubits and $\theta$ to subset $\overline{T}$ of size $n$. Then she measures her qubits in basis $\theta$ to produce a string $x$, and sends $\theta$ to $B$.

\item \textit{Post-processing}: $A$ and $B$ engage in some protocol using the strings $x$ and $\theta$, and $\widehat{x},\widehat{\theta}$ restricted to positions in $\overline{T}$.







\end{enumerate}



}

\begin{lemma}\label{lemma:min-entropy}
Consider the protocol in~\cref{fig:epr-protocol}. Let $n \geq m/2$. For any subset of $I \subset [n]$ of size $t$, let $\mathsf{wt}(I)$ be the number of positions in $I$ that $\theta$ and $\widehat{\theta}$ differ, and let $x_I$ be the string $x$ restricted to positions in $I$. Then for any $\epsilon > 0$, $x_I$ has quantum min-entropy (see definition in \cref{subsec: quantum min entropy}) at least $\mathsf{wt}(I) - \epsilon t$ conditioned on $B$'s view and on $x_{\overline{I}}$, except with probability $\negl(kt^2/n^2)$.
\end{lemma}

\begin{proof} (Sketch) We argue for the case where the strings $\widehat{\theta},\widehat{x}$ returned by $B$ are both the all-zeros strings; all other possibilities can be handled by applying the same arguments after an appropriate change of bases. Now consider the (purified) joint state $\ket{\psi_{\mathsf{A},\mathsf{B}}}$ of $A$ and $B$ in the middle of step 5, after $A$ has restricted her state to $n$ qubits. The check at the beginning of step 5 is essentially establishing that $A$'s part of $\ket{\psi_{\mathsf{A},\mathsf{B}}}$ is close to the all zeros state $\ket{0}^{\otimes n}$. Indeed, applying \cite[Theorem 3]{C:BouFeh10} (plus analysis in \cite[Appendix B.4]{C:BouFeh10} bounding the error probability of the corresponding classical sampling strategy) with some $\delta > 0$ shows that, conditioned on $A$ not aborting after this check, $A$'s part of the state is within trace distance $\negl(k \delta^2)$ of a superposition of states with Hamming weight at most $\delta n$. That is, we can assume that the state $\ket{\psi_{\mathsf{A},\mathsf{B}}}$ is a superposition of vectors that only contain at most $\delta n$ 1s among the $n$ positions in $\mathsf{A}$. Now, letting $\delta = \epsilon' t/n$ for a small enough constant $\epsilon' > 0$ and applying \cite[Corollary 1]{C:BouFeh10} shows that the conditional min-entropy (conditioned on $R$'s portion of the state) of $x_I$ is at least $\mathsf{wt}(I) - \epsilon t$.



\end{proof}

